DLoRA: Distributed Parameter-Efficient Fine-Tuning Solution for Large Language Model

To enhance the performance of large language models (LLM) on downstream tasks, one solution is to fine-tune certain LLM parameters and make it better align with the characteristics of the training dataset. This process is commonly known as parameter-efficient fine-tuning (PEFT). Due to the scale of LLM, PEFT operations are usually executed in the public environment (e.g., cloud server). This necessitates the sharing of sensitive user data across public environments, thereby raising potential privacy concerns. To tackle these challenges, we propose a distributed PEFT framework called DLoRA. DLoRA enables scalable PEFT operations to be performed collaboratively between the cloud and user devices. Coupled with the proposed Kill and Revive algorithm, the evaluation results demonstrate that DLoRA can significantly reduce the computation and communication workload over the user devices while achieving superior accuracy and privacy protection.

==> sections/8_relatedwork.tex <==
\section{Related Works}
In this section, we introduce three types of related works and illustrate the difference between them and the DLoRA system.
\paragraph{Offloading System} With the size of models getting bigger, computing only relying on edge devices is becoming more challenging. Offloading systems aim to offload part of the heavy computation burden to a cloud server. DLoRA differs from all the offloading systems by picking the personalized information-related parameters and constraining the execution to be only on edge devices.
\paragraph{Federated Learning} Federated Learning targets to build a "super" model with the aggregation of different users' data without leaking the information. However, supermodels can't guarantee the performance of models on personalized data. Nevertheless, even the model that is trained with Federated Learning algorithms can't be executed directly on edge devices, which makes the computation burden unavoidable.
\paragraph{LLM Compression} The inclusion of compression mechanisms can substantially enhance the efficiency of PEFT methods. The commonly used methods in model compression are model pruning and model quantization. 

